An optically pumped magnetic gradiometer for the detection of human biomagnetism

We realise an intrinsic optically pumped magnetic gradiometer based on non-linear magneto-optical rotation. We show that our sensor can reach a gradiometric sensitivity of 18 $\text{fT}/\text{cm}/\sqrt{\text{Hz}}$ and can reject common mode homogeneous magnetic field noise with up to 30 dB attenuation. We demonstrate that our magnetic field gradiometer is sufficiently sensitive and resilient to be employed in biomagnetic applications. In particular, we are able to record the auditory evoked response of the human brain, and to perform real-time magnetocardiography in the presence of external magnetic field disturbances. Our gradiometer provides complementary capabilities in human biomagnetic sensing to optically pumped magnetometers, and opens new avenues in the detection of human biomagnetism.

==> notes.tex <==
%\citep{Wens23} theory paper about various types of sensors for MEG \citep{Stolz21} SQUID gradiometers explained in detail \citep{Koga13} or \citep{Koga13b}compares various MEG systems including axial gradiometers - here are many graphs showing that axial gradiometers are better but the paper is only cited once...  \citep{Clancy21} \citep{Marhl22} compares axial in the squid configuration 

%\acomm{The phase of the net resonance shifts only with the gradient field $b$, however, since we track the changes of overlapped resonances, the observed frequency shift of the gradiometer is $\omega (B_0\pm b/2)$. The signal}

%In figure \ref{fig:overlapping} (a) we show a simplified layout of this scheme and the precession frequency observed for two cells. When equal-but-opposite-sign bias fields $\vec{B}_{0}$ are applied to two cells, the atoms within each will precess at the same frequency. Figure \ref{fig:overlapping} (b) shows the application of both a homogeneous external field $\vec{B}_{ext}$ and a small, spatially varying gradient $\vec{b}$; both cells experience the common field, whilst only cell 2 will measure the gradient. Generating counter-propagating bias fields in the two cells will mean that a common field will accelerate precession in one cell and decelerate it in the other cell by the same amount, resulting in no net frequency change. The small gradient field is only experienced by cell 2 and is not cancelled by cell 1, resulting in a net frequency shift. This is the operational principle of our gradiometer. 

%We apply a fixed bias field across the cells and then sweep the modulation frequency of the laser current. This generates in-phase and quadrature signals from the atoms, which have an associated phase between the two. To put each cell under the same bias field means to overlap the resonances. In order for this to work, we include a half-wave plate between the cells. This will cause a 180 degree phase shift of the signal produced by the second cell on the lock-in amplifier. Without the waveplate, the signal from the second cell is negative, meaning overlapping the signals from both cells would destructively interfere, resulting in no signal. With the waveplate in place, the individual resonances constructively add, causing a single high amplitude resonance. A simple depiction of this phase is shown in \ref{fig:overlapping} (c). Here the phase signal produced by both cells is shown. The external field $\vec{B}_{ext}$ will shift the phase signal from the two cells in opposite directions. This will cancel out any net shift caused by $\vec{B}_{ext}$, and the only remaining shift will be produced by the gradient in cell 2, $\vec{b}$. 

%Tracking this gradient is the same as tracking the magnetichttps://www.overleaf.com/project/64bf97cfb65881422d906ca1 field in conventional frequency-modulated NMOR magnetometry. We employ a phase-locked loop (PLL) to continually update the laser modulation to match the precession frequency of the atoms, ensuring they are always at the maximum resonant response. 

%The fundamental limit to this method is when the splitting of resonances occurs, this can be due either to a large gradient or magnetic field. The latter is more likely, where a common field larger than the resonance widths ($\Gamma$) no longer overlaps the resonances, and the PLL will fail to track a single central frequency. For larger fields such as this, the optical scheme still allows for the sensor to be operated as a magnetometer, by simply not applying a bias field to one of the cells. 

%commercial sensors $10-20~$fT$/\sqrt{\text{Hz}}$ \citep{Osborne2018, Alem23}

%Currently, the most advanced technology employing atomic spins is based on optically pumped neutral atoms \citep{Budker2007} as they offer the most straightforward experimental implementation. %\lcomm{Rewrite this sentence, sounds more like an advertisement and is not factually true; SQUIDs are more advanced in terms of realised performance.}
%The intrinsic optical subtraction of the homogenous background fields results from setting the bias field in each cell in opposite direction.   
%a half-waveplate rotates the light’s polarization direction 180
%The intrinsic gradiometer described in this paper is able to 


%An all-optical intrinsic scalar magnetic gradiometer based on cesium atoms has been developed by \citep{Zhang20}. The gradiometer noise level decreased by a factor of 3.3 compared to the single-cell magnetometer and was able to detect MCG signals in a magnetically noisy environment such as an office. 
%To achieve good measurement of the magnetic field we cannot continuously pump the atoms with a laser at resonance, as it will cause polarisation phase decoherence of the atomic ensemble . To rectify this issue, we employ synchronous optical pumping, or frequency modulation (FM) of the laser diode \citep{Acosta2006}. Tuning the laser away from resonance with the atomic transition allows us to modulate the laser in and out of this transition. Modulating the laser diode with a frequency equal to even multiples of the Larmor frequency allows us to retain the phase coherence of the atoms, resulting in an oscillatory solution that evolves as 2$\Omega_L$. In this experiment, we drive at double the Larmor frequency to stimulate resonance at 0 and $\pi$ radians. Using FM NMOR, we get a coherent population of magnetically sensitive atoms. Placing these atoms in a constant field allows us to measure $\Omega_L^0$, and tracking $d\Omega$ is possible with the use of lock-in detection. We then use a control loop to set the laser frequency to match that of the atoms, which has two distinct effects. Tracking this frequency change allows us to measure the magnetic field, and injecting it into the laser diode will realise a closed-loop system in which the atoms themselves dictate the new frequency of precession. This process is critical to the success of NMOR magnetometers, as it enables a high dynamic range of measurement.
%Gradiometer in practice
%Putting two cells in series in the optical scheme allows two resonances to be measured in one oscillator frequency sweep. In this setup, the spectral response from the atoms will result in one line-shape with a positive voltage response, and another with a negative response. Overlapping these two spectra, by applying the same field to both cells, would result in zero signal. To rectify this issue a $\frac{\lambda}{2}$ waveplate is placed between the two cells, in order to shift the phase of the second cell's signal by 180 degrees, resulting in two positive signals from both cells. The result is an additive superposition of lineshapes, which share a single central frequency that can be tracked. As well as the waveplate, we place the two cells under equal but opposite fields. This will cause a cancellation of homogeneous fields, and the measurement of a gradients. So long as no large transient magnetic fields occur during measurement, the only measured quantity is the magnetic gradient. 

%To probe the response of the gradiometer's rejection to external noise, we measured $\overline{R}$ under three different conditions. The first is the 'normal operating condition' described above, where $\Gamma$ was fixed at 55~Hz. In the second condition we introduced a 100nT external DC homogeneous field across the two cells, denoted $B_e$. With $B_e$ fixed, we compensate for this field with the on-board bias coils, to return to the central resonance frequency of 1.5~kHz. We then run the test as normal. This second condition demonstrates the ability of the gradiometer to compensate for external fields and still perform adequately. In the third condition we turned off the DC offset and instead increased the laser power delivered to the cells. This widened the resonance width to $\Gamma$ = 75~Hz. Under this condition the larger resonance means that the range of overlap between the two resonance signals is increased, resulting in greater rejection $\overline{R}$ over a larger range of $\delta$B.



%As expected, an increase in noise amplitude results in a decrease in rejection, this is shown clearly in the inset plot of figure \ref{fig:Rejection}. The increasing field strength causes a splitting of the resonances, and with this increase in splitting we see a reduction in the rejection. Setting $B_e$ to both 0nT and 100nT show comparable rejection performance. 

% \textcolor{red}{To get data for figure 3:
% - applied white noise generated with the arbitrary signal generator to drive the current source controlling solenoid coils. we set the noise bandwidth to 100 Hz and were changing the noise amplitude in the range 0.5 to 5nT (yellow and pink line in the inset of fig 3 - set A and B see below) or 0.5 to 10nT green line (set C) in the inset of fig 3
% - for each noise amplitude we recorded 10 sets of 3 second traces with cell 2 as magnetometer, then processed data in the following way:
% steps 1-3
% 1 - we did FFT on each trace, 2- we turn FFT to Power in dB (20log10), 3 - average 10 of the power spectra)
% Do the same with the gradiometer (steps 1-3), 
% - We subtract final gradiometer spectrum from the magnetometer spectrum to get the R.
% We did steps 1-3 with frequency resolution of 0.33 Hz}

% \textcolor{red}{We repeat it for  3 SETS of conditions:
% SET A - pink line in the inset - 0nT $B_e$, best width of the resonance to get best sensitivity - 55Hz
% SET B - yellow line. width is still 55Hz but we add 100nT DC offset  to the homogeneous noise $B_e$ and we correct for this offset by changing bias field in cell 2 to put the resonance in 1.5 kHz range for the magnetometry set, and by adjusting both bias fields in the gradiometer and  overlapping the grad signal at 1.5khZ, then we vary the noise amplitude in the 0.5 nT to 5nT range as above and repeat steps 1-3
% SET C- Green - we return the offset of $B_e$ at 0 nT again but we increase the power of the laser beam to create resonance that has  75 Hz width. we change now  amplitude of the noise in the range 0l5 to 10 nT and repeat steps 1-3}

% \textcolor{red}{Now to do the main plot in figure 3, that shows  the R over applied noise range we select 2 traces from set A (the  at 0.9 nT dark green trace and at 5.1 nT - pink trace). then we smoothen the data - we average every 4 points in the range 1 to 99 hz, ignoring 0 hz, 50 hz and 100 hz)
% to plot the inset - each point in set A B and C is averaged across all frequencies (1-99) excluding 50 Hz. So like averaging the whole dark green line or the pink line makes one point in the inset}
% %\gcomm{why noise amplitude? what the hell is this? aren't we measuring magnetic fields? what is a noise amplitude? what are the units? } detected with a magnetometer and gradiometer respectively, in the 0-110 Hz band. For every signal strength \gcomm{this is unclear, what do we do exactly? we apply a uniform magnetic field that varies sinusoidally, we change its amplitude, we record the aplitude of the signal generate by the sensor??}. For each value of \gcomm{...what?}, we collect 10 three-second traces with our sensor working in two configurations: i) the standard gradiometer configuration, ii) the magnetometer configuration, in which the bias field in one of the two cells is switched off. We then compute the logarithm of the ratio between the traces acquired in the two configurations, providing us with $R$. 

%The TFR does shows signal activation consistent with brain activity. The brain dynamics however, are not very clear meaning there must be something causing the decline in amplitude measured. The. The second issue has been a systematic issue during the human trials. In the benchtop shield, the sensor is mounted in a static mount, but despite this, it requires near-daily adjustment of the screws in order to keep the mirror aligned, the response maximised, and the phase between in-phase and quadrature components around 0. This alignment issue was many more times enhanced in the MSR, in which people move in and out of the mount, pushing and pulling on the sensor, inevitably requiring offset adjustment. Atop this, as mentioned in section \ref{sec:performance}, in the current setup there is no way to well-optimise the CMRR whilst the sensor is in the MSR, meaning that it was most likely not in the best working window during human trials. 

%The other issue is the scalp-sensor distance, which can be reduced by redesigning the bias coils and heating unit to become more compact, which is possible as the current bias coils are designed for larger cells. Both of these effects will significantly increase the viability of the sensor for human testing. Many of the controls during the optimisation of the sensor was left to manual adjustment, which is a time consuming process. Implementing a software solution to optimise the sensor is possible and would improve the time between human trials. The addition of modulation on the bias coils would allow for the testing of common-mode rejection within the MSR, which was previously only possible in the bench-top shield. These are solvable engineering issues, and does not effect the conclusion so far: the physics of using NMOR as method to measure gradients is clearly effective. 

% In conclusion, we show the viability of single-beam NMOR as a simple intrinsic method for sensitively measuring gradients whilst rejecting homogeneous magnetic fields. The sensor performed well in the lab environment, with 'benchtop' figures showing both common-mode rejection and sensitivity that were at the levels required for measuring biomagnetic gradients. In human trials the measurements of these fields were possible, with both MEG and MCG recordings producing results. Reproduction of the auditory evoked response was completed, as well as live heart-beats during transient magnetic field drifts. These measurements were, however, compromised by both the mechanical design of the sensor and the lack of sensor optimisation within the MSR. Rigidity and scalp-sensor distance were two factors causing both a decline in amplitude and an increase in noise. A rigid redesign of the sensor, and the optimisation of parts to minimise the scalp-sensor distance will allow the gradiometer to better measure these small fields. Including on-sensor self-calibration in which cell heating and bias fields are controlled programatically, maximizing SNR and CMRR, will further improve the ability of the sensor to work with human participants within the MSR. Further investigations into ... ..understanding best working parameters (temperature, laser power, overlapping) will be completed. Beyond this, an improved sensor will be used for new neuroscientific paradigmns enabled by NMOR gradiometry, such as the fast recovery times and dynamic range required for concurrent MEG with transcrainial magnetic stimulation in which large pulses of magnetic fields are used to induce currents within the brain. 

%Further work :
    %Rigidity & standoff
    %Investigate physics

%The sensor has both good sensitivity as well as the ability to reject common fields, proving NMOR as a physical mechanism to intrinsically measure small-amplitude gradients. Sensitivity can be increased with better tuning of the PLL, noiseless laser heating and better control of bias fields. The value of the rejection as well as its response to $\delta$B can be improved by increasing the laser power, at the cost of sensitivity due to larger resonance width. The bias coils were able to compensate for 100nT external field, keeping the resonance frequency between 1-2kHz. Stronger current drivers for the bias coils will be able to compensate for higher fields. Another option would be to use these external fields themselves as the bias field, and using the on-board coils to compensate for small field differences so that overlap could be achieved. This could move the sensor towards lower shielding environments, or ambient operation at the cost of a higher resonance frequency, provided that the external field is relatively homogeneous. Adapting and automating the CMRR-maximising protocol (applying a common known sinusoidal field, whilst adjusting heating and the bias field) to the sensor-level, perhaps on the bias coils themselves, would allow the sensor to self-optimise when performing the following biomagnetic measurements in the magnetically shielded room which contains no external coils.     

%HARRY
    % DEFINITIONS AND SHORTHAND
    %
